GeometrySticker: Enabling Ownership Claim of Recolorized Neural Radiance Fields

Remarkable advancements in the recolorization of Neural Radiance Fields (NeRF) have simplified the process of modifying NeRF's color attributes. Yet, with the potential of NeRF to serve as shareable digital assets, there's a concern that malicious users might alter the color of NeRF models and falsely claim the recolorized version as their own. To safeguard against such breaches of ownership, enabling original NeRF creators to establish rights over recolorized NeRF is crucial. While approaches like CopyRNeRF have been introduced to embed binary messages into NeRF models as digital signatures for copyright protection, the process of recolorization can remove these binary messages. In our paper, we present GeometrySticker, a method for seamlessly integrating binary messages into the geometry components of radiance fields, akin to applying a sticker. GeometrySticker can embed binary messages into NeRF models while preserving the effectiveness of these messages against recolorization. Our comprehensive studies demonstrate that GeometrySticker is adaptable to prevalent NeRF architectures and maintains a commendable level of robustness against various distortions. Project page: https://kevinhuangxf.github.io/GeometrySticker/.

==> rubbish.tex <==
%As shown in~\Fref{fig:algo_overriew}, given a binary message ${\mathbf{M}}$ with length $N_{b}$, we create a minibatch of geometry values $\mathbf{\Sigma}$ with the same size of $N_{b}$, and a MLP message encoder $\Theta_{\mathbf{M}}$ to encode the message into watermarked geometry values:

%Instead, we propose a message-sticking strategy to add geometry perturbation on the established NeRF, which can keep the NeRF network weights unchanged to ensure scalability for different NeRF baselines. Our GeometrySticker uses the Learnable CDF to select key points as a sparse geometry representation to add on the NeRF geometry. 

% Directly embedding messages into the geometry values $\sigma$ leads to noticeable distortions. 
% To ensure minimal visual alteration on the renderings, the message encoding strategy should refrain from embedding across all the geometry values.
%As shown in \Fref{fig:algo_overview}, 
%given a binary message ${\mathbf{M}}$ with length $N_{b}$, we first use message feature encoder $\Theta_m$ to encode the messages $\mathbf{M}$ and the 3d points coordiniates $\mathbf{x}$ into message feature $\mathbf{f_{M}} = \Theta_{\mathbf{M}$.
% we create a minibatch of 3D points with the same size of $N_{b}$ for message summation. associated with geometry values $\mathbf{\Sigma}$ and the confidence values $\mathbf{\Gamma}$. A MLP message encoder $\Theta_{\mathbf{M}}$ to encode the message into watermarked geometry values:

%\begin{equation}
%\mathbf{\Tilde{\Sigma}} = \mathbf{\Sigma} + \mathbf{\Gamma} \Theta_{\mathbf{M}}(\mathbf{\Sigma}, \mathbf{M} ).
%\label{eq:encode_watermark}
%\end{equation}
%where $\mathbf{\Gamma}$ is confidence values for selecting key points corresponding to the geometry values minibatch, and $\mathbf{\Tilde{\Sigma}}$ is the minibatch of watermarked geometry values.

%Since we embed the message into watermarked geometry values, which is independent and disentangled with the color prediction. Thus, the final rendered pixel is estimated based on the watermarked geometry values by:
%\begin{equation}
%\Tilde{C}(\mathbf{r})=\sum_{i=1}^N\exp(-\sum_{j=1}^{i-1}\Tilde{\sigma}_j\delta_j)(1-\exp(-\Tilde{\sigma}_i\delta_i))\mathbf{c}_i,
%\label{eq:watermarked_color_predict}
%\end{equation}
%where $\delta$ is the distance between adjacent sample points, $\mathbf{\Tilde{\sigma}}$ is the watermarked geometry value from $\mathbf{\Tilde{\Sigma}}$, and $c$ is NeRF predicted color.

% \noindent\xiufeng{\textbf{Messages decoding.}} \xiufeng{We design decoders for single image messages decoding and multi-view messages decoding. 
% We use the VGG16 as the backbone network for the single image decoding to extract features and connect with a linear layer for the message decoding. 
% To utilize temporal features between multiple rendering images, we utilize a 3D convolutional block which takes the rendering images $X \in \mathbb{R}^{T \times W \times H \times D}$ as input to extract the temporal features. The 3d convolutional block kernel size $K=11$ and is followed by a batch normalization and TanH activation. Based on this architecture, the message decoder can fully utilize the features from the multi-images from the NeRF renderings to enhance the message decoding further.}

\noindent\textbf{Extracting messages from sticker.} 

Our optimization is to optimize about three parts: the selected geometry values $\Psi_\beta(\sigma)$, message feature encode $\Theta_{m}$, message fusion module $\Theta_{f}$, a message decoder $D_m$ that can decode binary messages from rendered images, and a watermark classifier $C_m$ that can recognize the watermarked renderings. The classifier and the decoder both use a VGG16 network to extract image features, and utilize linear layers to make message prediction and classification prediction.  Our goal in optimization is to make the binary messages invisible in rendered contents, and then such binary messages can effectively be extracted via the message decoder. Then, the message decoder is optimized via the binary entropy loss as follows: 
\begin{equation}
    \mathcal{L}_{msg}=-\log\left(D_m(I_{w})\right)-\log\left(\mathbf{M})\right),
    \label{eq:message_loss}
\end{equation}
where $\mathcal{L}_{msg}$ is the message loss, $I_{w}$ is the watermarked rendered image and $\mathbf{M}$ is the ground truth message. 
Meanwhile, we also optimize the watermark classifier to recognize the watermarked contents:
\begin{equation}
    \mathcal{L}_{cls}=-\log\left(C_m(I_{w})\right)-\log\left(1 - C_m(I_{o})\right),
    \label{eq:message_loss}
\end{equation}

We then optimize the watermarked image similar to the original image by using MSE loss
\begin{equation}
    \mathcal{L}_{cont} = \|I_{w} - I_{o}\|_2^2,
    \label{eq:content_loss}
\end{equation}
where $\mathcal{L}_{cont}$ is the content loss to optimize the learnable SDF parameter $\beta$, the message encoder $\Theta_{m}$ and fusion module $\Theta_{f}$ so that the rendered watermarked image $I_w$ is similar to the original image $I_o$. The final total loss is estimated by:
 \begin{equation}
     \mathcal{L}_{total}=\mathcal{L}_{cont} + \mathcal{L}_{msg} + \mathcal{L}_{\text {sparse }}
     \label{eq:total_loss}
 \end{equation}

% The vanilla NeRF uses frequency positional encoding to transform the input coordinates and viewing direction with two cascaded MLP layers. The first MLP layer is for density prediction with 2 hidden layers of 64 channels and the second MLP layer is for color prediction with 3 hidden layers of 64 channels. InstantNGP utilizes a hash encoding as the positional encoding and two compact MLP layers based on the tiny-cuda implementation. The first density prediction MLP has 1 hidden layer with 64 channels and the following color prediction MLP layer has 2 hidden layers with 64 channels. The TensoRF contains a separate density grid and a feature grid for geometry and color prediction. 
